Texture Synthesis with Recurrent Variational Auto-Encoder

We propose a recurrent variational auto-encoder for texture synthesis. A novel loss function, FLTBNK, is used for training the texture synthesizer. It is rotational and partially color invariant loss function. Unlike L2 loss, FLTBNK explicitly models the correlation of color intensity between pixels. Our texture synthesizer generates neighboring tiles to expand a sample texture and is evaluated using various texture patterns from Describable Textures Dataset (DTD). We perform both quantitative and qualitative experiments with various loss functions to evaluate the performance of our proposed loss function (FLTBNK) --- a mini-human subject study is used for the qualitative evaluation.

==> contributions.tex <==
\hl{(to do, according to github requirements)}\\
The following are the contributions made by each team member:

\begin{enumerate}
\item Ahmed Taha: 
\item Moustafa Meshry:
\item Sachin Grover:
\item Rohan Chandra:
\item Kyungjun Lee:
\end{enumerate}

==> figures_tex/quantitative.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
	  \includegraphics[scale=0.4]{figures/logs_l2_loss.png}
      \caption{Training using L2 loss}
	\end{subfigure}
    ~
	\begin{subfigure}[b]{0.4\textwidth}
	  \includegraphics[scale=0.4]{figures/logs_cross_ent_loss.png}
      \caption{Training using cross-entropy loss}
	\end{subfigure}

	\begin{subfigure}[b]{0.4\textwidth}
	  \includegraphics[scale=0.4]{figures/logs_fb_loss.png}
      \caption{Training using filter-bank loss}
	\end{subfigure}
    ~
	\begin{subfigure}[b]{0.4\textwidth}
	  \includegraphics[scale=0.4]{figures/logs_vgg_loss.png}
      \caption{Training using VGG loss}
	\end{subfigure}

	\caption{Tracking different losses during training.}
	\label{fig:quantitative}
  \end{figure*}


